JenGAN: Stacked Shifted Filters in GAN-Based Speech Synthesis

Non-autoregressive GAN-based neural vocoders are widely used due to their fast inference speed and high perceptual quality. However, they often suffer from audible artifacts such as tonal artifacts in their generated results. Therefore, we propose JenGAN, a new training strategy that involves stacking shifted low-pass filters to ensure the shift-equivariant property. This method helps prevent aliasing and reduce artifacts while preserving the model structure used during inference. In our experimental evaluation, JenGAN consistently enhances the performance of vocoder models, yielding significantly superior scores across the majority of evaluation metrics.

==> figure/figure_jengan.tex <==
\begin{figure}[!hbt]
\setlength{\textfloatsep}{0pt}%
    \setlength{\textfloatsep}{0pt}%
    \setlength{\intextsep}{0pt}
    \centering
\includegraphics[width=0.95\linewidth]
{figure/figure}
\caption{JenGAN method overview}
\label{fig:jengan_figure}
\end{figure}

==> figure/frequency_domain.tex <==
\begin{figure}[!ht]
\setlength{\textfloatsep}{0pt}%
    \setlength{\textfloatsep}{0pt}%
    \setlength{\intextsep}{0pt}
    \centering
\begin{tikzpicture}
\begin{axis}[
    % title={Plots of frequency domain space when $\delta$ is varying},
    xlabel={$f$},
    % ylabel={$X(f)$},
    xmin=-0.5, xmax=0.5,
    ymin=-0.13, ymax=0.3,
    xtick={-0.5,-0.25,0,0.25,0.5},
    ytick={-0.125,0,0.125,0.25},
    legend style={
                at={(1.05,0.5)},
                anchor=west,
                % text = blue,
                },
    legend cell align={left},
    reverse legend,
    % legend pos=south west,
    grid style=dashed,
    width=0.8\linewidth,
]

\addplot[
    domain=-0.5:0.5,
    samples=100,
    color=blue,
    style={very thick},
    ]
    {0.25 - x^2};
\addlegendentry{$\delta=0.0$}

\addplot[
    domain=-0.5:0.5,
    samples=100,
    color=orange,
    style={very thick},
    dotted,
    ]
    {(0.25 - x^2) * cos(0.5*deg(pi*x))};
\addlegendentry{$\delta=0.25$}

\addplot[
    domain=-0.5:0.5,
    samples=100,
    color=red,
    style={very thick},
    dotted,
    ]
    {(0.25 - x^2) * cos(1*deg(pi*x))};
\addlegendentry{$\delta=0.5$}

\addplot[
    domain=-0.5:0.5,
    samples=100,
    color=violet,
    style={very thick},
    dotted,
    ]
    {(0.25 - x^2) * cos(1.5*deg(pi*x))};
\addlegendentry{$\delta=0.75$}

\addplot[
    domain=-0.5:0.5,
    samples=100,
    color=green,
    style={very thick},
    dotted,
    ]
    {(0.25 - x^2) * cos(2*deg(pi*x))};
\addlegendentry{$\delta=1.0$}

\end{axis}
\end{tikzpicture}
\caption{Plots depicting the frequency domain space of $X(f)$ as $\delta$ varies, with $\delta = 0.0, 0.25, 0.5, 0.75, 1.0$. Near zero in frequency space, variations in $\delta$ do not lead to significant changes. However, as the magnitude of $f$ increases, changes in $\delta$ induce noticeable fluctuations.}
\label{fig:frequency_domain}
\end{figure}
